Declarative Recursive Computation on an RDBMS, or, Why You Should Use a Database For Distributed Machine Learning

A number of popular systems, most notably Google's TensorFlow, have been implemented from the ground up to support machine learning tasks. We consider how to make a very small set of changes to a modern relational database management system (RDBMS) to make it suitable for distributed learning computations. Changes include adding better support for recursion, and optimization and execution of very large compute plans. We also show that there are key advantages to using an RDBMS as a machine learning platform. In particular, learning based on a database management system allows for trivial scaling to large data sets and especially large models, where different computational units operate on different parts of a model that may be too large to fit into RAM.

==> handling-very-large-queries.tex <==
\section{Handling Very Large Query Plans}

The recursive specifications of the last section address the problem of how to succinctly specify complicated recursive
computations so as to avoid any control flow that may force bad decisions upon the underlying system.  Yet the question 
remains: How can the very complex computations associated with such specifications be executed?

To demonstrate the very high complexity of such a computation, consider the feed-forward network learner given in Section 3, and
the SQL code:

\begin{SQL}
EXECUTE (
  FOR i IN 0...99:
    EXPORT (ERRORS [i][9]) TO 'errors' + i + '.csv'

  FOR l in 1...8:
    MATERIALIZE (WEIGHTS[99][l])
)
\end{SQL}

\noindent
As a result of this computation, 100 iterations of training will be completed.
Each of the prediction errors incurred during those 100 training iterations will be written to a text file. 
Also, the complete set of weights learned at the end of the 100 iterations will be saved to the database, so that they can be 
used to make predictions, or improved upon by subsequent training.

The obvious way to execute this computation would be to start with the 108 different tables that are requested by
this execution, and then completely
unroll the recursion, computing the complete set of tables that would need to be computed in order to supply the 108 user-requested
tables.  The complete set of dependencies between those tables
could then be compiled into a relational algebra computation, and then optimized and executed using a (mostly)
standard, RDBMS-like engine.

The problem with this is that the resulting graph would be huge.  Each of the 100 training iterations for an eight-layer network
consists of 584 relational algebra operations, including 56 joins and 15 aggregations.
Thus, 100 training iterations results in a query plan having 56,900 operations in all.
No existing RDBMS engine could possibly optimize and execute such a complex computation.  Analyzing and optimizing the plan itself
is a 
particular bottleneck.  Many different approaches to building query optimizers have been suggested over the years, but all of them
assume a plan that is at most a few dozen operations in size.  None of them are meant to scale into plans consisting of
thousands of operations.  Further, the situation here is unique in that the application
is very unforgiving.  Doing the wrong thing 
(such as deciding to materialize the errors being back-propagated through the links in a deep net) can result in 
a computation plan that can bring down the system.

\vspace{5 pt}
\noindent \textbf{Frame-based execution.}
To deal with this, an obvious idea is to partition the query plan into \emph{frames}, and to optimize and execute those frames 
independently.  
A frame is simply a small sub-computation of the entire unrolled recursive computation.  To execute the overall plan, 
one frame is optimized and executed, \textcolor{red}{and its output materialized}.  Then a second frame is
optimized and executed, and  \textcolor{red}{its output materialized}. Frames are only optimized and executed once all of their inputs
have been materialized.  This is repeated until the entire computation is complete. 

Frame-based computation
is an attractive option because as long as each frame is small enough that an existing query optimizer and execution engine
handle the frame, the RDBMS optimizer and engine need not be modified in any way.  Further, this iterative execution results in 
an engine that resembles engines that perform re-optimization during runtime \cite{kabra1998efficient}, 
in the sense that frames are optimized 
and executed only once all of their inputs have been materialized.  Accurate statistics can be collected on those inputs, 
meaning that classical problems associated with errors propagating up a query plan can be avoided.

However, the problem with this approach is that cutting the computation into frames necessarily commits the system to a certain
set of choices regarding the implementation and execution of the plan.  Specifically, a cut across a long between one operation
and the next means that the data flowing across that operation must be materialized.  Hence, in a sense we are back to where
we started in Section 3 of the paper, where the iteration-based computation forced a programmer to materialize data in order
to communicate between iterations, and the amount of data to materialize was debilitating.
Here, we are again forced to materialize data in order to communicate between frames.
A poor choice of cut can bring us back to where we were in Section 3, where it does not matter how well we optimize and execute
each frame, because the cost of moving data between frames is debilitating.

Hence, in the remainder of the paper, we turn our attention to a central question: How can we efficiently cut a very large, 
unrolled computation into a set of frames, in such a way that the overall execution time is not significantly greater than
had we somehow been able to optimize and execute the entire computation as a whole?

%\begin{figure}[h]
% \centering
% \includegraphics[width=9cm]{graph.pdf}
% \caption{One iteration of a neural network. Red represents the forward-propagation, purple the back-propagation and blue the weight update}
%\end{figure}



==> intro.tex <==
\section{introduction}

Most popular tools for building machine learning (ML) algorithms  
(such as TensorFlow \cite{tensorflow}, Caffe2 \cite{caffe2}, and PyTorch \cite{pytorch}) are essentially numerical optimization engines
bolted on top
of a compute engine.  In the ideal case, to use such a tool, the
programmer specifies a model in the form of a loss function, 
and the tool generates a numerical optimization procedure (typically, gradient decent) by automatically differentiating
the model.  
This optimization procedure is then run on top of the system's compute engine.

\vspace{5 pt}
\noindent
\textbf{Parameter Servers for Machine Learning.}
Most widely-used ML algorithm-generation tools (such as TensorFlow \cite{tensorflow})
use a so-called \emph{parameter server} \cite{Smola:2010, Li:2014}
as the underlying distributed compute engine for executing automatically-generated algorithms.

A parameter server is essentially a distributed
key-value store.  In a parameter server,
a set of machines are designated as \emph{servers}. Servers typically store fragments of the model, addressable
via a unique key.  The remainder of the machines are designated as workers.  \emph{Workers} repeatedly
load a small portion of the training
data, request some relevant part of the model, use the data to update the part of the model, and then push the
updated model to the servers.

In the common case that
the numerical optimization procedure to minimize the loss function is generated automatically and the end user is 
more skilled in mathematics than in writing Big Data codes, 
it is desirable for the compute engine to run the numerical optimization procedure well, 
no matter how large or small the data set and model, and no matter how many machines are used to run the
computation, or the amount of resources (CPU and RAM) available on each machine.
To learn a model twice as quickly, just requisition twice the machines (and hence twice the CPUs/GPUs) and run the same code.
This is the ``one implementation, any model/data size and compute hardware''
ideal.

Unfortunately, this is not the reality for today's distributed deep learning tools.
It is true that a parameter server can be used to implement any distributed computation---just as 
a tool such as MPI \cite{gropp1996high}
can be used to implement any distributed computation---but the problem is that getting many distributed computations
to work on top of a parameter server will 
typically require a large amount of human effort.
For anything other than relatively simple computations,
a programmer must manually
break the computation into discrete units and then make choices about which servers serve which data,
which workers run which computations, which machines workers and servers are housed on, how to synchronize the servers
and workers, etc.  The result is that in practice, parameter servers such as TensorFlow are most often
used to execute computations on a single machine.
For distributed learning,
parameter servers
are typically used for running asynchronous, stochastic gradient descent algorithms \cite{bottou2010large} in the simple
case where the model is small enough to be easily broadcast in its entirety to each worker. 
The various workers each have a small subset of the data, which they
use to update the model, and then asynchronously (or synchronously)
send their updates back to the parameter server.  This
is the so-called \emph{data parallel} implementation.
In practice data parallel implementations are preferred because they are easy.  Each processing unit performs the same
computation over different subsets of the data.

In contrast, in many situations, a \emph{model parallel} implementation---where various workers work on different parts of 
a huge model---would be desirable.  Depending upon the application, the model may be so large that it cannot fit into the RAM
of any particular machine and so model parallelism is required. 
Or, the model may be complicated and difficult to compute, and as we will argue, data parallelism
is limited in its ability to speed convergence of distributed gradient descent algorithms.  Model parallelism can help.

Unfortunately, various claims both in the folklore and in research papers, parameter servers \emph{do not} support easy 
model parallelism, where ``easy'' model parallelism would insulate a programmer from the details of the distributed implementation,
the same way in which SQL insulates a database programmer from the details of how a distributed query is executed.
In the ideal case, the gradient descent algorithm automatically generated by the ML platform's front end would automatically
run well on any model/data size and compute
hardware.  However, this is far from the reality of the situation.

\vspace{5 pt}
\noindent
\textbf{Adapting RDBMS Technology for ML.}
In contrast, the goal of ``one implementation, any model/data size and compute
hardware'' coincides almost perfectly
to the relational database management system (RDBMS) concept of \emph{data independence}, which has been a guiding principle of
RDBMS design since their inception in the 1970's.
To support data independence, databases are fundamentally based upon the declarative programming paradigm \cite{codd1970relational}:
the programmer (or algorithm generator) specifies
what he/she/it wants, and not how to compute it, and the computation is automatically optimized to match the data and hardware.
We will argue that this makes an RDBMS a great platform for distributed machine learning.

Besides the principle of data independence, RDBMSs have many other characteristics to recommend their use as a replacement for
a parameter server as the compute platform for distributed ML computations.
Databases are fast, robust, distributed query optimization is now well-understood and highly effective \cite{chaudhuri1998overview}.
It is not an accident that competing distributed compute platforms
such as Spark \cite{zaharia2010spark} (which now promotes the use of relational-style DataFrames \cite{Armbrust:2015} and DataSets \cite{datasets} interfaces) 
are beginning to look more like a parallel RDBMSs.

Our central thesis in this paper is that it makes little sense to reinvent the wheel---that ideas such as declarative programming
and data independence have made RDBMSs so successful make a lot of sense for distributed machine learning as well.
We will show that it is possible to express deep learning computations in a few lines of SQL, and have those computations 
automatically parallelized in a truly model-parallel way.
We will argue that there is nothing unique
about modern ML computations that make them particularly amenable to the key-value style of programming
required by a parameter server.  In fact, such computations look at lot like the classical analytics queries that have been 
successfully evaluated by distributed RDBMSs for the past two decades. 
Hence, tools such as TensorFlow should be using RDBMS-like backends, rather than those based upon parameter serves.

However, there are a couple of reasons that a
modern RDBMS' cannot be used out-of-the-box as a platform for most large-scale machine learning algorithms.  
Crucially, such systems lack sufficient
support for recursion. In deep learning, for example, it is necessary to ``loop'' through the layers
of a deep neural network, and then ``loop'' backwards through the network
to propagate error and update the model.
All of this is repeated within another ``loop'' that repeatedly runs the forward-backward passes.
Such ``looping'' could be expressed declaratively via recursive dependencies among tables, but RDBMS 
support for recursion is typically limited (if it exists at all)
to computing fixed-points over sets--specifically with an eye towards computing transitive closures \cite{aho1979universality}.
And crucially, even if one adds sufficient support for recursion to an RDBMS, there is the problem that
the ``query'' plan for a typical deep-learning computation may run to tens of thousands of operators, which no 
existing RDBMS optimizer is going to be able to handle.

\vspace{5 pt}
\noindent
\textbf{Our Contributions.}
In this paper, 
we consider exactly how database support for recursion should be enhanced to handle large-scale machine learning
computations, and then address the question of how a typical query optimization framework can be modified so that
it can handle the massive query plans that result from complicated recursive computations.  We implement our ideas on
top of SimSQL, which is a prototype distributed RDBMS that is specifically designed to handle large-scale statistical
computation.

For two distributed deep learning problems (a feed-forward neural network and an implementation of Word2Vec \cite{word2vec:NIPS2013, mikolov2013efficient}) we show that 
declarative SimSQL codes of the kind that could be auto-generated by an ML algorithm-generation tool 
outperform corresponding TensorFlow parameter server implementations, and scale to huge model sizes that are
beyond the capabilities of the implementations that ship with TensorFlow.  This is despite the fact that SimSQL has
the performance handicap of being a
Java-based prototype RDBMS implemented on top of MapReduce.  
A high-performance RDBMS would likely do even better.
We also show that a distributed LDA implemented on top of SimSQL generally scales better and outperforms 
the same implementation on top of TensorFlow's parameter server (as well as Apache Spark).  

Taken together, these results call into question the current practice of developing state-of-the-art machine learning
platforms on top of a distributed parameter server, and instead suggest that a more RDBMS-like backend is perhaps a more
suitable choice.


